Dynamic collision avoidance for multiple robotic manipulators based on a non-cooperative multi-agent game

A flexible operation of multiple robotic manipulators in a shared workspace requires an online trajectory planning with static and dynamic collision avoidance. In this work, we propose a real-time capable motion control algorithm, based on non-linear model predictive control, which accounts for static and dynamic collision avoidance. The proposed algorithm is formulated as a non-cooperative game, where each robot is considered as an agent. Each agent optimizes its own motion and accounts for the predicted movement of surrounding agents. We propose a novel approach to formulate the dynamic collision constraints. Additionally, we account for deadlocks that might occur in a setup of multiple robotic manipulators. We validate our algorithm on a pick and place scenario for four collaborative robots operating in a common workspace in the simulation environment Gazebo. The robots are controlled by the Robot Operating System (ROS). We demonstrate, that our approach is real-time capable and, due to the distributed nature of the approach, easily scales to an arbitrary number of robot manipulators in a shared workspace.

==> Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> sections/simulation_results.tex <==
\section{Results} \label{sec:results}
\subsection{Simulation setup and controller parametrization}
The multi-robot setup is built in a robotic simulation environment \highlight{Gazebo} \cite{koenig2004design} with four simulated collaborative robotic manipulators UR3 from \highlight{Universal Robots}. \highlight{Gazebo}  provides an interface to control the robots using the Robot Operating System (ROS) \cite{ros}. In this paper we use the distribution \highlight{ROS Melodic}. The communication is established through the ROS action client to the \highlight{Universal Robot} ROS driver. The ROS interface allows that the simulation environment \highlight{Gazebo} can easily be replaced by an experimental test bed. The four model predictive controllers run in parallel on a computer with an Intel $8700$k at $3.7$ GHz using $32$ GB RAM under Ubuntu 16.04. The coordinator is running on the same computer and communicates the computed optimal trajectories with the controllers via the TCP/IP protocol.\\

The control algorithms are implemented in \highlight{Matlab} using \highlight{CasADi} \cite{Andersson2019} for setting up the non-linear program for the DMPCs. The merit of \highlight{CasADi} is its automatic differentiation capability, i.e., \highlight{CasADi} computes the first and second order derivatives of the cost function and constraints using automatic differentiation. We use the interior point solver \highlight{IPOPT} \cite{wachter2006implementation}  to solve the optimization problem and apply \highlight{MA27} \cite{hsl2007collection} to solve the underlying linear system. We set the maximum number of iterations to $100$ and an acceptable tolerance of $10^{-4}$. In addition, \highlight{CasADi} is instructed to pre-compile the optimization problems using just-in-time compilation. We choose a sampling time of $T_\textrm{s}=0.1 \ \unit{s}$ and a horizon length of $N_p = 15$, which means a prediction time of $1.5 \ \unit{s}$.  \\

In this work we validate our motion control algorithm for a pick and place scenario comprising $M=4$ robotic manipulators with $N=6$ degrees of freedom each. Each robot is approximated by $8$ line segments and $5$ ellipsoids, resulting in $40$ conceivable constraints for each pair of manipulators. That means overall $120$ conceivable constraints per local DMPC. However, geometrically it is impossible to position four robots in a setup, where all constraints need to be taken into account, i.e. robots standing in a diagonal could only collide with their wrist links and robots standing next to each other will never reach the basis and shoulder links of the other one. Therefore, only $26$ instead of $120$ conceivable collision constraints, for each DMPC, need to be considered. Additionally, $2$ static collision constraints to avoid collision with the table are taken into account. \\

The four robots and the objects are placed on top of a table of a height $z_\textrm{T} =0.85 \ \unit{m}$. The positions of the basis of the four collaborative robotic manipulators in the workspace, omitting the $z$-coordinate, are as follows 
\begin{align*}
    \mathbf{p}_1^B =& (0.0 ,\quad 0.0), \qquad \qquad \mathbf{p}_2^B = (0.744 ,\quad 0.0), \\
    \mathbf{p}_3^B =& (0.744 ,\quad 0.744), \qquad \mathbf{p}_4^B = (0.0 ,\quad 0.744 ). 
\end{align*}
The four objects are placed in such a way that multiple collisions between the robots and a deadlock can occur. Therefore the positions of the objects are chosen as
\begin{align*}
    \mathbf{O}_1 =& (0.3 ,\quad 0.18 ), \qquad  \mathbf{O}_2 = (0.4 ,\quad 0.3 ), \\
    \mathbf{O}_3=& (1.0 ,\quad 0.6 ), \qquad \ \ \mathbf{O}_4 = (0.3 ,\quad 0.42 ). 
\end{align*}

The task for each robot $i$ is to grasp an object $\mathbf{O}_i$ and bring it to the robot's initial configuration pose. The validation scenario consists of two consecutive tasks, which are to move to the object, grasp it and move back to the initial configuration and release the object, which are shown in Figure \ref{fig:gazebo_snips} (a,d). The initial positions of the robotic manipulators' end effectors in Cartesian space are
\begin{align*}
    \mathbf{p}_1^0 =& (-0.4, \quad 0.2015, \quad 0.035),\\
    \mathbf{p}_2^0 =& (1,2 ,\quad 0.2, \quad 0.035), \\
    \mathbf{p}_3^0 =& (0.45 \quad 0.59, \quad 0.035), \\ \mathbf{p}_4^0 =& (-0.3, \quad 0.5184, \quad 0.035).
\end{align*}

The weighting matrices of the DMPCs are chosen as  
\begin{align*}
    \mathbf{Q}_i^\textrm{x}&=\textrm{diag}(1,1,1,0.2,0.2,0.2,1,1,1,0.2,0.2,0.2),\\
    \mathbf{Q}^\textrm{f}_i&=10 \cdot \mathbf{Q}_i^\textrm{x},\quad 
    \mathbf{R}_i^\textrm{u}=0.1 \cdot \mathbf{I}^{6 \times 6} ,\quad    \mathbf{R}_i^\textrm{d}=15 \cdot  \mathbf{I}^{6 \times 6}. 
\end{align*}
Joint positions and velocities of the three wrist links are penalized less to allow for a greater freedom of motion. The joint velocities and accelerations are limited to $\pi$. The parameters for the deadlock algorithm are set as follows 
\begin{equation}
         \varepsilon=10^{-2}, \quad \delta = 2\cdot10^{-2}, \quad d_\textrm{s}=0.25.     
\end{equation}

\subsection{Input delays of closed-loop non-linear model predictive control}
The number of active dynamic collision constraints summarized in equation \eqref{eq:dynamic_collision_k} change dynamically, as not all possible collisions can occur at a time step $k$. The number of active collision constraints considerably affects the computation times of the non-convex optimization problem $\eqref{eq:DMPC}$, which can be seen in the Table \ref{tab:compTimes_table} for maximum computation times $T_\textrm{c,max}$. Indeed, $T_\textrm{c}$ might even be greater than the sampling time $T_\textrm{s}$ and therefore the optimal control input $\mathbf{u}^{* \; 0}$ can not be obtained immediately. \\
\renewcommand{\arraystretch}{1.3}
\begin{table}[h!]
    \centering
    \begin{tabular}{|c||c|c|c|}
    \hline
    Controller Type & $T_\text{c,min}$ [ms] & $T_\text{c,max}$ [ms] & $T_\text{c,mean}$ [ms] \\[5pt]
    \hline
    Centralized MPC & 120 & 670.5 & 232.9\\ [5pt]
    \hline 
    Distributed MPC $R_1$ & 26.9 & 185.6 & 64.8 \\ [3pt]
    Distributed MPC  $R_2$ & 22.9 & 128.8 & 38.7\\ [3pt]
    Distributed MPC  $R_3$ & 21.1 & 188.9 & 32.2\\ [3pt]
    Distributed MPC $R_4$ & 20.1 & 103.3 & 36.1\\ [3pt]
    \hline
    \end{tabular}
    \caption{Minimum, maximum and mean computation time values of distributed and centralized MPC.}
    \label{tab:compTimes_table}
\end{table}

The larger the sampling time $T_\textrm{s}$, the smaller the influence of the computation time $T_\textrm{c}$ on the DMPC. However, the sampling time cannot be increased arbitrarily, otherwise tunneling will occur. For this reason, we followed the approach of Grüne and Pannek \cite{grune2017nonlinear} to account for the non-negligible computation times. As the maximum computation time is $T_\textrm{c,max} < 2 \cdot T_\textrm{s}$, we solve the DMPC every $2 \cdot T_\textrm{s}$, still with a sampling time $T_\textrm{s}$ within the optimization.\\

In the following, we illustrate the approach for a single joint $q \in \mathbb{R}$ and maximum computation times greater than $T_\textrm{s}$ i.e., $T_\textrm{c,max} > T_\textrm{s}$ holds. At time $t_k$, a new measurement $q^k$ is received from the manipulator. Due to the computation time $T_\textrm{c}$, a new optimal control input is not available at time $t_k$. The robot is provided the optimal control input from the last optimization step for time $t_k$ until $t_k + T_\textrm{c,max}$.  Figure \ref{fig:input_delays} illustrates this concept for $T_\textrm{c,max} > T_\textrm{s}$ and the green line designates the optimal control inputs $[u^{*\;1} \ u^{*\;2}]$. Simultaneously, at time $t_k$, the state $q^k$ is extrapolated into the future by integrating the manipulators dynamics $f(q(t),u(t))$
\begin{equation}
    \hat{q}^k=q^k + \int_{t_k}^{t_k+T_{c,\text{max}}} f(q(t),u(t)) dt.
\end{equation}
With $\hat{q}^k$ as the initial condition, the optimization problem \eqref{eq:DMPC} is solved so that a new trajectory and control input is available at the latest at time $t_k + T_\textrm{c,max}$. At time $t_k+T_\textrm{c,max}$ the obtained optimal control input $u^{*\;0}$, illustrated by red in Figure~\ref{fig:input_delays}, is sent to the robot. At time event $t_{k+2}$ the DMPC receives a new measurement $q^{k+2}$ and the procedure is repeated.  We follow Krämer et al.~\cite{Kraemer2020} and obtain $T_\textrm{c,max}$ via a moving average filter over past observed delays.
%The first optimal input $u^*_{0,t_n}$ is applied at time $T_s - T_{c,\text{max}}$, where the time $T_{c,\text{max}}$ is a constant time event at which the optimal inputs are applied. The second
\begin{figure}
    \centering
%    \includegraphics[width=0.49\textwidth]{graphics/delayed_input.eps}
     \begin{overpic}[width=0.42\textwidth]{graphics/delayed_input_2Ts.eps}
        \put(10,10){$t_k$}
        \put(47,10){$t_{k+1}$}
        \put(83,10){$t_{k+2}$}
        \put(98,10){$t$}
        \put(32,10){$T_{c,\text{max}}$}
        \put(28,3){$T_s$}
        \put(65,3){$T_s$}
        \put(9,60){$q^k$}
        \put(60,65){$\hat{q}^k$}
        \put(46,72){$q^{k+1}$}
        \put(83,65){$q^{k+2}$}
   %     \put(30,60){$q_{m}$}
   %     \put(36,58){\color{black}\vector(1,-0.8){4}}
        \put(26,42){$u^{* \; 1}$}
        \put(52,34){$u^{* \; 2}$}
        \put(70,35){$u^{*\;0}$}
        \put(-8,70){$q, u$}
      \end{overpic}
    \caption{Compensation of computation times $T_\textrm{c,max} \geq T_s$ for non-linear model predictive control.}
    \label{fig:input_delays}
\end{figure}

\subsection{Validation of the motion algorithm}
\begin{figure}[h!]
   \centering
    \begin{subfigure}{0.40\textwidth}
        \hspace{6mm}
        \includegraphics[width=\textwidth]{graphics/workspace_trajectory_legend.pdf}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphics/workspace_trajectory_case15_new.pdf}
    \end{subfigure}
    \caption{Trajectory of robots' end effectors in the workspace.}
    \label{fig:workspace_trajectory}
\end{figure}
\begin{figure}[h!]
\begin{tabular}{cc}
  \includegraphics[width=40mm]{graphics/initial_config.png} &   \includegraphics[width=40mm]{graphics/collision_avoidance_four.png} \\
(a) Initial configuration & (b) Collision avoidance  \\
at $t=0 \ \unit{s}$ & at $t=2.8 \ \unit{s}$ \\ [6pt]
 \includegraphics[width=40mm]{graphics/first_deadlock.png} &   \includegraphics[width=40mm]{graphics/final_config.png} \\
(c) Deadlock detection & (d) Final configuration \\
 at $t=11.5 \ \unit{s}$ &  at $t = 65 \ \unit{s}$ \\ [6pt]
\end{tabular}
\caption{Selected time frames from the simulation environment \highlight{Gazebo}.}
\label{fig:gazebo_snips}
\end{figure}
With the compensation of input delays at hand, we turn our attention to the validation of our motion algorithm. The setup of four robots is chosen in a way to show the efficacy of the previously introduced approaches for dynamic collision avoidance and deadlock detection. Figure \ref{fig:workspace_trajectory} shows the trajectory of the four robots' end effectors in the workspace. The robots start at positions $\mathbf{p}^0_1$ for Robot $1$ illustrated as black line, $\mathbf{p}^0_2$ for Robot $2$ illustrated as red line, $\mathbf{p}^0_3$ for Robot $3$ illustrated as blue line and $\mathbf{p}^0_4$ for Robot $4$ illustrated as green line. The arrow tip on the right border of Figure \ref{fig:workspace_trajectory} indicates from which side the four robots in Figure \ref{fig:gazebo_snips} are observed. The initial and final configuration of the robots, which are identical, are shown in Figure \ref{fig:gazebo_snips}a and \ref{fig:gazebo_snips}d, respectively. The trajectories to the objects $\mathbf{O}_1$, $\mathbf{O}_2$, $\mathbf{O}_3$ and $\mathbf{O}_4$ are depicted as solid lines and the trajectories back to the final target are illustrated by dashed lines in Figure \ref{fig:workspace_trajectory}. The arrows indicate in which direction the robots are moving along their trajectories. \\

The depicted trajectories show, that each robot chooses a different path to return to its initial position compared to the outward trajectory. Collision avoidance between the robots can be especially seen for Robot $3$, whose object is placed outside the shared workspace with the robot's initial configuration inside the workspace. 
At time $t=2.8  \ \unit{s}$, Robot $3$ avoids Robot $2$ by moving over it. This can be observed in the $3$D simulation in Figure \ref{fig:gazebo_snips}b or in Figure~\ref{fig:joint_stateq4} where the joint angle $q_4(t)$ of Robot $2$ show noticeable deflections. This moment is indicated by crosses in the workspace trajectory in Figure \ref{fig:workspace_trajectory}. A closer look at Figure \ref{fig:costFunc} shows that Robot $3$ avoiding Robot $2$ is accompanied by a slight increase of its cost function. During the same time range, Robot $1$ also chooses another path in order to avoid a collision with Robot $4$. A less strong deviation of the joint angle $q_4(t)$ can be seen in Figure~\ref{fig:joint_stateq4}. \\

Objects $\mathbf{O}_1$, $\mathbf{O}_2$ and $\mathbf{O}_4$ are positioned in close proximity in the middle of the common workspace. Therefore, it is impossible for the manipulators $1$, $2$ and $4$ to pick up the three objects simultaneously without causing a collision. With this case, we illustrate how the robots solve such a dilemma in a non-cooperative game, as every agent acts egoistically to achieve its own best possible benefit. Robot $1$ manages to reach the target before the other robots. The other two robots $2$ and $4$ come in close proximity to robot $1$ and prevent robot $1$ from grasping the object effectively resulting in a deadlock at time $t=11.5 \ \unit{s}$. The former can be seen in the $3$D simulation in Figure \ref{fig:gazebo_snips}c. 
%Thereafter, the other two robots prevent each other from grasping the objects effectively resulting in a deadlock. At time $t=40.1 \ \unit{s}$ the deadlock is detected between the manipulators $2$ and $4$ by the coordinator, see Figure \ref{fig:gazebo_snips}c. 
As Robot $1$ is closest to its target, robots $2$ and $4$ are deactivated, i.e., the coordinator sets $\gamma_2 = 0$ and $\gamma_4 = 0$, until Robot $1$ has grasped the object. Due to repulsive forces of the deactivated robots, Robot $1$ pushes Robot $2$ aside to grasp its object, which can be seen in the full line along the dashed line in Figure \ref{fig:workspace_trajectory}. Robot $2$ is more affected as it is closer to Robot $1$ and after the deadlock is resolved Robot $2$ returns back to grasp its object.   
The cost function of Robot $1$ rises at time $t=25.6  \ \unit{s}$, where the robot receives the next task. At the same time, the coordinator resets $\gamma_2 = 1$ and $\gamma_4 = 1$ and the deadlock is resolved.  Notice, that Robot $3$ executes its task unaffected by the deadlock and its resolution.\\
%\begin{figure}[h!]
%    \centering
%    \begin{subfigure}{0.40\textwidth}
%            \hspace{5mm}
%            \includegraphics[width=\textwidth]{graphics/workspace_trajectory_legend.pdf}
%    \end{subfigure}
%    \begin{subfigure}
%        \begin{tabular}{cc}
%              \includegraphics[width=0.49\textwidth]{graphics/joint_states_q1.pdf} &   \includegraphics[width=0.49\textwidth]{graphics/joint_states_q2.pdf} \\
%           (a) Joint angle $q_\textrm{Base}(t)$ & (b) Joint angle $q_\textrm{Shoulder}(t)$ \\
%          [6pt]
%            \includegraphics[width=0.49\textwidth]{graphics/joint_states_q3.pdf} &  
% \includegraphics[width=0.49\textwidth]{graphics/joint_states_q4.pdf} \\
%         (c) Joint angle $q_\textrm{Elbow}(t)$ & (d) Joint angle $q_\textrm{Wrist,$1$}(t)$ \\
%            [6pt]
%       \end{tabular}
%    \end{subfigure}
%\caption{Joint angles of four robot manipulators.}
%\label{fig:joint_angles}
%\end{figure}

\begin{figure}[h]
   \centering
    \begin{subfigure}{0.40\textwidth}
        \hspace{6mm}
        \includegraphics[width=\textwidth]{graphics/workspace_trajectory_legend.pdf}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphics/joint_states_q4_new.pdf}
    \end{subfigure}
    \caption{First wrist position of four robotic manipulators.}
    \label{fig:joint_stateq4}
\end{figure}

The cost function values show exactly when the robot receives a new target. High cost function values indicate that a robot received a new target and is far away from it, which can be seen in Figure \ref{fig:costFunc}. \\

\begin{figure}[h]
   \centering
    \begin{subfigure}{0.40\textwidth}
        \hspace{6mm}
        \includegraphics[width=\textwidth]{graphics/workspace_trajectory_legend.pdf}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{graphics/costFunction_case15_new.pdf}
    \end{subfigure}
    \caption{Cost function of four robotic manipulators.}
    \label{fig:costFunc}
\end{figure}

In order to draw conclusions about real-time capabilities of the derived algorithm, computation times have to be considered. In Figure \ref{fig:comp_times} computation times over real-time can be seen for each robot. The computation times rise significantly, when most of the collision constraints are active. This can be seen for the time range $0.1  \ \unit{s} \leq t \leq 2.7  \ \unit{s}$ highlighted in Figure \ref{fig:comp_times}. Further, computation times rise again at time $25.6 \ \unit{s}$, when all four robots are in the shared workspace, i.e. when Robot $3$ moves to its final pose and Robot $1$ grasps its object and moves to its final target. In that case, the robots have to avoid each other and the computation times of robots $1$ and $2$ reach another peak. \\ %During the deadlock, which happens at time range $40.1  \ \unit{s} \leq t \leq 48  \ \unit{s}$, indicated by the third highlighted range in Figure \ref{fig:comp_times}, the computation times remain stable as only collision avoidance between the last wrist joints for robots $2$, $3$ and $4$ are active.  \\

\begin{figure}[h]
   \centering
    \begin{subfigure}{0.40\textwidth}
        \hspace{6mm}
        \vspace{-2.5mm}
        \includegraphics[width=\textwidth]{graphics/workspace_trajectory_legend.pdf}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{graphics/computation_times_case15_new.pdf}
    \end{subfigure}
    \caption{Computation times of four robotic manipulators.}
    \label{fig:comp_times}
\end{figure}

Last but not least, we discuss the computational cost and, therefore, real-time capabilities of our approach. To get an impression of the the speed-up, we compare our approach to a more traditional, centralized MPC. As the cost function $J$ for the centralized approach, we choose the sum of the individual cost functions of the robots, i.e.\
\begin{equation}
    J = J_1 + J_2 + J_3 + J_4.
\end{equation}
For the collision avoidance in the centralized setting, the robots are approximated with line segments and ellipsoids to ensure a comparability of the results. Table \ref{tab:compTimes_table} showed minimum, maximum and mean computation times for each robot. As can be seen from the table, even the minimum computation time for the centralized approach lies above the sampling time $T_\textrm{s}=100 \ \unit{ms}$. The maximum computation time is almost $7$ times higher than the sampling time. Compared to the centralized MPC, minimum computation times of the distributed MPC lie considerably below the sampling time and the maximum times can be compensated by the procedure explained before. A careful comparison of computation times for centralized and distributed MPC leads to the following conclusion: A speed-up of a factor $4$ can be achieved by choosing the distributed MPC over the centralized approach. This is to be expected, since the optimization problem for the centralized MPC is split into four optimization problems with one fourth of the original size. These results indicate that the distributed approach leads to real-time capable computation times which cannot be provided by the centralized MPC. \\

